Channel-Recurrent Autoencoding for Image Modeling

Despite recent successes in synthesizing faces and bedrooms, existing generative models struggle to capture more complex image types, potentially due to the oversimplification of their latent space constructions. To tackle this issue, building on Variational Autoencoders (VAEs), we integrate recurrent connections across channels to both inference and generation steps, allowing the high-level features to be captured in global-to-local, coarse-to-fine manners. Combined with adversarial loss, our channel-recurrent VAE-GAN (crVAE-GAN) outperforms VAE-GAN in generating a diverse spectrum of high resolution images while maintaining the same level of computational efficacy. Our model produces interpretable and expressive latent representations to benefit downstream tasks such as image completion. Moreover, we propose two novel regularizations, namely the KL objective weighting scheme over time steps and mutual information maximization between transformed latent variables and the outputs, to enhance the training.

==> Implementations.tex <==
\section{Implementation Details}\label{sec:detail-training}
\paragraph{Modification of VAE-GAN objective from~\cite{larsen2015autoencoding}.} We empirically found that reconstructing the last convolutional layer of the discriminator to maximize $\E_{q_\phi (z|x)}\big[\log p_{\theta}(x|z)\big]$ as proposed in~\cite{larsen2015autoencoding} leads to more instability in training comparing to reconstructing at the pixel-level. Hence, throughout our work, we reconstruct at the pixel level for both VAE-GAN and {\LSTMVAEGAN}. 

\paragraph{Data Augmentation.} For Birds and CelebA, random horizontal flipping is used during training as data augmentation. For LSUN, random cropping and horizontal flipping are used.

\paragraph{Optimization.} Our models are optimized with ADAM~\cite{kingma2014adam}, where we set $\epsilon=1\times 10^{-8}$,  $\beta_1 = 0.9$, $\beta_2 =0.999$. 
%
For the discriminator, we use a variation of ADAM with additional thresholding~\cite{faces}: if the classification accuracy of the discriminator for a batch consisting of half real and half fake images is over $90\%$, we do not update the model parameters of the discriminator. 

\paragraph{Initial Learning Rate.}  For Stage1 models, Birds has initial learning rate $0.0003$, CelebA $0.003$ for {\VAEGAN} and $0.001$ for {\LSTMVAEGAN}, LSUN $0.0003$ for {\VAEGAN} and $0.0001$ for {\LSTMVAEGAN}. For all Stage2 networks, we use $0.0002$ as initial learning rate. 

\paragraph{Objectives.} Recall the VAE objective:
\begin{equation}
\Loss_{\mathrm{VAE}} = \underbrace{-\E_{q_\phi (z|x)}\big[\log p_{\theta}(x|z)\big]}_{\Loss_{\mathrm{recon}}} + \underbrace{D_{\mathrm{KL}} ( q_\phi (z|x) \Vert p(z) )}_{\Loss_{\mathrm{prior}}} \geq -\log(p(x)).
\end{equation}
%
Conventionally, for RGB images, $p_{\theta}(x|z)$, a diagonal {\mvg}, is assumed to have fixed variance $\sigma$ and only the mean values are estimated which correspond to pixel values. 
%
We follow this convention and apply MSE loss at the pixel level, which we find effective even without feature-level reconstruction, and defer $\sigma$ to be adjusted through weighting the $\Loss_{\mathrm{prior}}$, i.e. the KL-divergence term, by introducing an additional hyperparamter $\alpha$. 
%
Recall that we weigh the KL-divergence term differently for different time steps when training {\LSTMVAE}, i.e. for the first 3 time steps with $\alpha_1$ and the rest $\alpha_2$. 
%
Moreover, the adversarial loss is weighted by hyperparameter $\beta$. Together, we have the following training objective for RGB images:
\begin{equation}
\Loss_{\mathrm{VAE}\text{-}\mathrm{GAN}} = \Loss_{\mathrm{recon}} + \alpha \Loss_{\mathrm{prior}} + \beta \Loss_{\mathrm{D}},
\end{equation}
%
where 
%
\[
\Loss_{\mathrm{D}} = -\log(D(x)) - \log(1-D(\mathrm{gen}(z))),  z\sim p(z), \text{ or } z\sim q_\phi (z|x).
\]
%
It is worth mentioning that the generated samples, which are decoded from $z$ sampled from the prior $p(z)$, and the reconstructed samples, which are decoded from $z$ sampled from the approximated posterior $q_{\phi}(z|x)$, are both used for training with adversarial loss. Specifically, a mini-batch for discriminator update is assembled with $50\%$ real examples (half), $25\%$ generated samples (a quarter) and $25\%$ reconstructed samples.
%when sampling from $z\sim p(z)$, the fake example is a generated sample and when sampling from $z\sim q_\phi(z|x)$ a reconstructed sample; a mini-batch for discriminator training is assembled with $50\%$ real examples (half), $25\%$ generated samples (a quarter) and $25\%$ reconstructed samples.
%
Also, note that $\Loss_{\mathrm{recon}}$ is divided not only by the batch size, but also by the channel, width and height of the images for implementation convenience, while $\Loss_{\mathrm{prior}}$ or $\Loss_{\mathrm{D}}$ are divided by the batch size only. This explains why the optimal $\alpha$ or $\beta$ values are considerably smaller than one.
%

\paragraph{$\alpha$ and $\beta$}
For Birds, {\VAEGAN} is trained with $\alpha = 0.0002$ and $\beta= 0.0125$ and {\LSTMVAEGAN} $\alpha_1=0.0003$, $\alpha_2=0.0002$ and $\beta=0.0125$; for CelebA, {\VAEGAN} is trained with $\alpha = 0.0003 $ and $\beta = 0.01$ and {\LSTMVAEGAN} $\alpha_1 = 0.0003$, $\alpha_2=0.0002$ and $\beta= 0.01$; for LSUN, {\VAEGAN} is trained with $\alpha = 0.0002$, $\beta = 0.025$ and {\LSTMVAEGAN} $\alpha_1 = 0.0003$, $\alpha_2 = 0.0002$, $\beta = 0.0125$. 
%\footnote{In our implementation, $\alpha=0.0003$ corresponds to $0.0003\times3\times64\times64\approx3.69$.} for celebA and Birds and progressively reduces it to $0.0002$ over time for {\LSTMVAEGAN} models.
%
%For $\beta$ values, CelebA works the best with $\beta = 0.01$ and Birds $\beta = 0.025$. 

\paragraph{MI Objectives.}
In the main text, for {\LSTMVAEGAN}, we introduce a regularization term based on maximization of mutual information between the generation $\tilde{x}$ and its sampled latent variable $z$. 
%
We now mathematically justify and illustrate the formulation of the auxiliary objective:
%
\begin{align*}
 I(z,\tilde{x}) &= H(z) - H(z|\tilde{x})\\
 &=\E_{\tilde{x}\sim p_\theta (x|z)}\left[\E_{\tilde{z}\sim p(z|\tilde{x})}\left[\log p(\tilde{z}|\tilde{x})\right]\right] + H(z)\\
 &\geq \E_{\tilde{x}\sim p_\theta (x|z)}\left[\E_{\tilde{z}\sim p(z|\tilde{x})}\left[\log q(\tilde{z}|\tilde{x})\right]\right] + H(z) \\ 
&= \E_{z\sim p(z), \tilde{x}\sim p_\theta (x|z)}\left[\E_{\tilde{z}\sim p(z|\tilde{x})}\left[\log q_\psi (\tilde{z}|\tilde{x})\right]\right] + H(z) \\
&= \E_{z\sim p(z), \tilde{x}\sim p_\theta (x|z)}\left[\log q_\psi (z|\tilde{x})\right] + H(z), \\
\end{align*}
where $q_\psi (\tilde{z}|\tilde{x})$ is a variational approximation to $p(\tilde{z}|\tilde{x})$, parametrized by a neural network which shares the same encoding path with the discriminator. 
%
The last equality transformation comes from Lemma 5.1 in~\citep{chen2016infogan}.  
%
Similarly as done in~\citep{chen2016infogan}, we bypass the optimization of $H(z)$ by treating it as a constant and leverage the reparametrization trick to sample from $z$. 
%
As in the case for the adversarial loss, when given the ground truth $x$, we sample $z$ from its approximated posterior $q_\phi (z|x)$, otherwise sample from prior $p(z)$.
%
Therefore, the overall objective for the auxiliary task becomes:
\[
\Loss_{\mathrm{MI}} = \E_{z\sim p(z), \tilde{x}\sim p_\theta (x|z)}\left[\log q_\psi (z|\tilde{x})\right] + \E_{x\sim X, z\sim q_\phi (z|x), \tilde{x}\sim p_\theta (x|z)}\left[\log q_\psi (z|\tilde{x})\right]
\]
%
Recall that in the case of RGB images, the formulation $p_\theta (x|z)$ estimates the mean of the Gaussian distribution while fixing variance.
%
Therefore, in practice, we do not perform additional sample from $p_\theta (x|z)$ but directly take the mean.
%
Also, we assume $q_\psi (z|\tilde{x})$ to be a diagonal {\mvg} with fixed $\sigma$. 
%
In this way, the auxiliary objective boils down to $L^2$ reconstruction of $z$ from $\tilde{x}$. 
%
Finally, as explained in the main text, we found empirically reconstructing $z$ does not work as well as reconstructing the transformed latent variable $u = \mathrm{LSTM}(z)$, thus we set the objective to be the latter. 
%
Now the overall objective for {\LSTMVAEGAN} becomes 
\begin{equation*}
\Loss_{\mathrm{VAE}\text{-}\mathrm{GAN}} = \Loss_{\mathrm{recon}} + \alpha_1 \Loss^{1}_{\mathrm{prior}} +  \alpha_2 \Loss^{2}_{\mathrm{prior}} + \beta \Loss_{\mathrm{D}} + \kappa \Loss_{\mathrm{MI}},
\end{equation*}
where for Birds, $\kappa = 0.02$, for CelebA, $\kappa = 0.01$ and for LSUN, $\kappa = 0.01$. 

\paragraph{Stage2 Objective.} The objective for the discriminator during Stage2 training is to maximize:
\begin{equation*}
\Loss_{D} = \mathbb{E}_{s \sim S} \left[\log (D(s) )\right] +   \mathbb{E}_{z \sim p(z), \tilde{x} \sim p_\theta(x|z)} \left[\log (1 - D(G(\tilde{x}))\right] + \mathbb{E}_{z \sim q_{\phi}(z|x), \tilde{x} \sim p_\theta(x|z)} \left[\log (1 - D(G(\tilde{x}))\right].
\end{equation*}
The loss for the generator is to minimize
\begin{gather*}
\Loss_{G} = \mathbb{E}_{z \sim p(z), \tilde{x} \sim p_\theta(x|z)} \left[\log (1 - D(G(\tilde{x}))\right] + \mathbb{E}_{z \sim q_{\phi}(z|x), \tilde{x} \sim p_\theta(x|z)} \left[\log (1 - D(G(\tilde{x}))\right] + \\
 \gamma  \mathbb{E}_{z \sim q_{\phi}(z|x), \tilde{x} \sim p_\theta(x|z)} \left[\| f(S(x)) - f(G(\tilde{x})) \|^2_2\right],
\end{gather*}
where $S(x)$ is the ground truth upsampled $x$ and $f$ represent feature extraction via some pre-trained deep CNNs, namely VGG11 for Birds and CelebA and ResNet50 for LSUN. For the experiments without perceptual loss, $\gamma = 0$, otherwise $\gamma = 1$ for Birds and CelebA, and $\gamma = 10$ for bedroom.

\paragraph{Image Completion Hyperparameters.} Recall the image completion objective:
\begin{equation}
\min_z  \;\big[\Vert\hat{x}\odot m - x\odot m\Vert_{2}^{2} + \label{completion} \gamma \log \mathcal{N}(z;0,\mathbf{I}) + \tau \log (1-D(\hat{x})\big].\nonumber
\end{equation}
%
We use $\gamma= 0.00001$ and $\tau = 0.003$.
\newpage
\iffalse
\section{Details of Network Architecture}
\label{sec:model}
This section describes the building blocks used to construct the networks in our experiments. 
%
Throughout this section, we adapt the following notations:
\begin{itemize}
\item $C^s_n$ refers to a convolutional layer with $n$ filters and stride $s$.
\item $D_n$ refers to a deconvolutional layer with $n$ filters; in our networks, deconv layers are of stride 2 and kernel size 4$\times$4.
\item $\mathrm{FC}_n$ refers to a fully-connected layer with $n$ filters.
\item $P^k$ refers to $k\times k$ pooling.
\item $\mathrm{LSTM}^t_{n}$ refers to a $T$-time-step LSTM with $n$ hidden units. 
\item $\BN$ refers to Batch Normalization.
\item $\relu$ refers to ReLU activation, $\cat$ CReLU activation and $\leaky$ Leaky ReLU activation with 0.1 slope. 
\end{itemize}
\subsection{Inference Feature Extractor Architecture} 
The following models are used to extract convolutional features for inference:
\paragraph{MNIST.} All convolutions are of 3$\times$3 kernel size except for the first one (5$\times$5). We have the following architecture: 
\begin{align*}
&C^2_{32} +\BN + \cat \to C^1_{64} +\BN + \leaky \to C^2_{64} +\BN + \cat \to C^1_{128} +\BN + \leaky  \\ 
&\to C^2_{128} +\BN + \cat \to C^1_{256} +\BN + \leaky
\end{align*}
\paragraph{CelebA 64$\times$64.} Again, all convolutions here are of 3$\times$3 kernel size except for the first one (5$\times$5):
\begin{align*}
&C^2_{32} +\BN + \cat \to C^2_{64} +\BN + \cat \to C^2_{128} +\BN + \cat \to C^1_{256} +\BN + \cat  \\ 
&\to C^1_{256} +\BN + \leaky \to C^1_{256} +\BN + \leaky
\end{align*}
\paragraph{CelebA and Birds 128$\times$128.} All convolutions here are of 3$\times$3 convolutional kernels except for the first and second conv layers (5$\times$5)
\begin{align*}
&C^2_{32} +\BN + \cat \to C^2_{64} +\BN + \cat \to C^2_{128} +\BN + \cat \to C^1_{256} +\BN + \cat  \\ 
&\to C^1_{256} +\BN + \leaky \to C^1_{256} +\BN + \leaky
\end{align*}
\subsection{Deconvolutional Network Architecture} 
The following architectures are used to generate images from latent representations $u$. 
\paragraph{MNIST.} All convolutions are of 3$\times$3 kernel size except for the one before Sigmoid (1$\times$1).
\begin{align*}
&D_{256} +\BN + \leaky \to C^1_{256} +\BN + \leaky \to D_{128} +\BN + \leaky \to C^1_{128} +\BN + \leaky  \\ 
&\to D_{64} +\BN + \leaky \to C^1_{64} +\BN + \leaky \to D_{32} +\BN + \leaky \to C^1_{32} +\BN + \leaky \\
& \to C^1_{1} +\BN + \leaky \to \mathrm{Sigmoid}
\end{align*}
\paragraph{CelebA and Birds.} All convolutions are of 3$\times$3 kernels except for the one before Tanh (1$\times$1).
\begin{align*}
&D_{256} +\BN + \leaky \to C^1_{256} +\BN + \leaky \to D_{128} +\BN + \leaky \to  D_{64} +\BN + \leaky  \\ 
&\to D_{32} +\BN + \leaky \to C^1_{3} +\BN + \leaky \to \mathrm{Tanh}
\end{align*}
\subsection{Inference Path and Latent Decoding}
Now we specify the architecture that connects the extracted CNN features to mean and variance estimations as well as that connects the sampled latent representations to the deconvolutional networks. 
\paragraph{standard VAE.} We flatten the convolutional features to 1-D vectors and apply fully-connected layers during inference. Similarly, we apply FC layers to transform $z$ to $u$ then reshape $u$ before going to deconvolution.
\begin{itemize}
\item mean inference: $\mathrm{FC}_{1024}$
\item variance inference: $\mathrm{FC}_{1024}$
\item decoding $z$: $\mathrm{FC}_{256\times 4 \times 4}$
\end{itemize}
\paragraph{{\convVAE}.} We replace FC layers from standard VAE with convolutional layers without flattening the convolutional variables:
\begin{itemize}
\item mean inference: $C^{1}_{64}$
\item variance inference: $C^{1}_{64}$
\item decoding $z$: $C^{1}_{256}$
\end{itemize}

%\paragraph{{\blockVAE}.} For variance, we slice the convolutional features into $T$ ($T=64$ for celebA and $T=8$ for MNIST) subsets along the channel direction, then connect each subset with an independent FC layer. Same with decoding $z$. Also, we add an additional element-wise addition to mean inference and after the FC layers for decoding path. 
%\begin{itemize}
%\item mean inference: $C^{1}_{64} - \mu_0$
%\item variance inference: $(\mathrm{FC}_{1024/T}) \times T$
%\item decoding $z$: $(\mathrm{FC}_{256\times 4\times 4/T}) \times T + %\mu_0$
%\end{itemize}
\paragraph{{\LSTMVAE}.} Similar to {\blockVAE}, but instead of FC layers, we use LSTM to connect the sliced subsets. For MNIST, we use FC layer instead of conv layer for mean inference path due to MNIST's simple content is more suitable for FC layer.
\begin{itemize}
\item mean inference: $C^{1}_{64} - \mu_0$ or $\mathrm{FC}_{1024} - \mu_0$ (MNIST)
\item variance inference: $\mathrm{LSTM}^8_{256}$
\item decoding $z$: $\mathrm{LSTM}^8_{256} + \mu_0$
\end{itemize}

\subsection{Discriminator}
For all VAE-GAN and {\LSTMVAEGAN} experiments, the following Discriminator architecture is used:
\begin{align*}
&C^2_{32} + P^2 + \relu + \mathrm{Dropout} \to C^2_{64} + P^2 + \relu + \mathrm{Dropout}  \\ 
&\to C^2_{128} + P^2 + \relu + \mathrm{Dropout} \to C^2_{128} + P^2 + \relu + \mathrm{Dropout} \\
&\to \mathrm{FC}_{512} + \mathrm{Norm(1)} + \mathrm{Dropout} + \relu + \mathrm{BD} + \mathrm{FC}_{1} + \mathrm{Sigmoid},
\end{align*}
where all conv kernels are of size 5$\times$5 except for the last one (3$\times$3), Dropout ratio $0.5$, Norm(1) refers to normalizing $L^2$ norm of the incoming vectors to 1 and BD refers to Batch Discrimination layer~\citep{salimans2016improved}. 

%\subsection{STL-10 Models}
%For STL-10, we closely follow the model presented by~\cite{denton2016semi}. Instead of using deterministic autoencoders, we replace it with standard VAE as another baseline and our {\LSTMVAE}. The latent dimension is $2048$ for all models and $T=8$ for LSTM.
\subsection{Mutual Information Maximizer}
For CelebA, we use the following architecture for mutual information maximization objective:
\begin{align*}
&C^2_{32} + P^2 + \relu + \mathrm{Dropout} \to C^2_{64} + P^2 + \relu + \mathrm{Dropout}  \\ 
&\to C^2_{128} + P^2 + \relu + \mathrm{Dropout} \to C^2_{128} + P^2 + \relu + \mathrm{Dropout} \\
&\to C^1_{64} + \mathrm{BD} + \mathrm{Leaky} + C^1_{64} + \mu,
\end{align*}
where the last conv layer has kernel 1$\times$1, the second to last 3$\times$3. 
For birds:
\begin{align*}
&C^2_{32} + P^2 + \relu + \mathrm{Dropout} \to C^2_{64} + P^2 + \relu + \mathrm{Dropout}  \\ 
&\to C^2_{128} + P^2 + \relu + \mathrm{Dropout} \to C^2_{128} + P^2 + \relu + \mathrm{Dropout} \\
&\to C^1_{64} + \mathrm{BD} + \mathrm{Leaky} + C^1_{64} + \mathrm{BD} + \mathrm{Leaky} \\
&\to \mathrm{FC}_{1024} + \mu, 
\end{align*}
where the last conv layer has kernel 1$\times$1, the second to last 3$\times$3.  

Note that in both cases, the maximizer shares the same encoding path with the discriminator up till convolutional layer. 
\newpage
\section{Variations of {\LSTMVAE} on MNIST experiments}
For MNIST, we integrate {\LSTMVAE} into various existing advanced training technique or model framework of VAEs to highlight its generalizability. 
%
Specifically, we utilize importance weighted autoencoder framework (IWAE)~\citep{burda2015importance} and variational hierarchical graphical models~\citep{ranganath2016hierarchical}.  

\vspace{-0.1in}
\paragraph{channel-recurrent importance weighted autoencoder.}
%
The $k$-sample importance weighting estimate of the log-likelihood provides a tighter bound than the variational lower bound of VAEs~\citep{burda2015importance}. Since the probabilistic formulation of {\LSTMVAE} doesn't change from that of VAEs, the extension to importance weighted autoencoder, which we refer a {\LSTMIWAE}, is straightforward:
%
\begin{equation}
\Loss_{\mathrm{\LSTMIWAE},k} = \mathbb{E}_{z_{i}\sim q_{\phi}(z|x)}\big[\log \frac{1}{k}\sum_{i=1}^{k}\frac{p_{\theta}(x,z_{i})}{q_{\phi}(z_{i}|x)}\big].\nonumber
\end{equation}
%

%
%where the prior and posterior are factorized as follows:
%


\paragraph{Hierarchical VAE and {\LSTMVAE}.} There are many ways to build hierarchical models via VAE framework. 
%
In our experiments, we follow the hierarchical graphical model presented in~\citep{tomczak2017vae}.
%
To spell out the inference and generation respectively, we have:
\begin{gather*}
p_{\theta}(x,z^{1},z^{2}) = p_{\theta}(x|z^{1},z^{2})p_{\theta}(z^{1}|z^{2})p(z^{2})\\
q_{\phi}(z^{1},z^{2}|x) = q_{\phi}^{2}(z^{2}|x) q_{\phi}^{1}(z^{1}|z^{2},x)
\end{gather*}
For {\LSTMVAE}, we apply channel-recurrency to both layers and keep the same hyperparamters as 1 layer {\LSTMVAE}.

\paragraph{Hierarchical crIWAE.} We can also seamlessly integrate the hierarchical model on top of importance weighted training with channel recurrency where the loss is written as follows:
%
\begin{equation}
\Loss_{\mathrm{\LSTMIWAE},k} = \mathbb{E}_{z_{i}^{1},z_{i}^{2}\sim q_{\phi}(z^{1},z^{2}|x)}\big[\log \frac{1}{k}\sum_{i=1}^{k}\frac{p_{\theta}(x,z_{i}^{1},z_{i}^{2})}{q_{\phi}(z_{i}^{1},z_{i}^{2}|x)}\big]\nonumber
\end{equation}
\newpage 
\fi
